Generating Detailed Character Motion from Blocking Poses

We focus on the problem of using generative diffusion models for the task of motion detailing: converting a rough version of a character animation, represented by a sparse set of coarsely posed, and imprecisely timed blocking poses, into a detailed, natural looking character animation. Current diffusion models can address the problem of correcting the timing of imprecisely timed poses, but we find that no good solution exists for leveraging the diffusion prior to enhance a sparse set of blocking poses with additional pose detail. We overcome this challenge using a simple inference-time trick. At certain diffusion steps, we blend the outputs of an unconditioned diffusion model with input blocking pose constraints using per-blocking-pose tolerance weights, and pass this result in as the input condition to an pre-existing motion retiming model. We find this approach works significantly better than existing approaches that attempt to add detail by blending model outputs or via expressing blocking pose constraints as guidance. The result is the first diffusion model that can robustly convert blocking-level poses into plausible detailed character animations.

==> prelim.tex <==
\section{Problem Description }
\label{prelim}

\subsection{Desiderata} Our system aims to perform automatic motion detailing in the animation blocking workflows, using both kinematic motion diffusion and physics tracking-based systems as detail-enhancing tools in a progressive detailing loop. The animator provides a set of \textit{K} blocking poses $\mathbf{x} \in \mathbb{R}^{J \times D}$, where \textit{K} is the number of blocking poses, and each pose is represented by a \textit{D}-dimensional feature of $J$ joints . When placed on the timeline of length \textit{F} frames, these sparse blocking poses yield an underspecified \emph{blocking animation}. We refer to all such incomplete animations as $\mathbf{X} \in \mathbb{R}^{F \times J \times D}$. Diffusion-based and physics-tracking-based operators convert $\mathbf{X}$ into a completed \emph{detailed motion} that adheres to the coarse structure of the blocking motion (e.g., it contains similar poses as the original blocking poses, at similar points in time, but not necessarily an exact match of either), while exhibiting realistic motion. We refer to any completion of $\mathbf{Y}$, where $\mathbf{Y} \in \mathbb{R}^{F \times J \times D}$.



\section{Preliminaries}
\subsection{Kinematic Motion Diffusion}

The core component in kinematic motion diffusion models is a denoising network, which is trained to progressively reverse the Markov noising process and recover a realistic, high-fidelity motion sequence $\mathbf{Y}$. In the forward process, each clean motion $\mathbf{Y}$ is gradually perturbed by Gaussian noise according to:
\begin{equation}
q(\mathbf{Y}_t \mid \mathbf{Y}) = \mathcal{N}(\sqrt{\alpha_t} \mathbf{Y}, (1 - \alpha_t) \mathbf{I}),
\label{eq:markov}
\end{equation}
where $\alpha_t \in (0,1)$ is a monotonically decreasing schedule over diffusion timestep $t$. Diffusion models can also incorporate additional information to condition generation. $I$ is trained to predict a clean motion $\mathbf{\tilde{Y}}_{0,t}$ given a noisy input $\mathbf{Y}_t$, diffusion timestep $t$, and a conditioning input $\mathbf{X}$, where $\mathbf{X}$ is an underspecified animation sequence. The objective is:
\begin{equation}
\mathcal{L} = \mathbb{E}_{\mathbf{Y}, t}\left[ \| \mathbf{Y} - I(\mathbf{Y}_t, t, \mathbf{X}) \|^2 \right].
\end{equation}
At inference time, the denoising network is applied iteratively to a sample of pure Gaussian noise, reversing the diffusion process step-by-step to generate a realistic motion sequence. 




==> relatedwork-OLD.tex <==



\subsection{Kinematic Motion Synthesis}

Classical methods such as Motion Graphs~\citep{kovar2002motion,arikan2002interactive,lee2002interactive} synthesize motion by traversing a dataset, typically guided by trajectory constraints.
%
\citet{holden2016deep} introduced a Variational Autoencoder (VAE) \citep{kingma2013auto} to learn a latent motion space, enabling intuitive editing and synthesis.
%
Building on this, \citet{petrovich2021actor,petrovich2022temos} adopted Transformer architectures~\citep{vaswani2017attention} to address action-to-motion and text-to-motion tasks.
%
Subsequent methods such as T2M~\citep{guo2022generating}, T2M-GPT~\citep{zhang2023generating}, and MotionGPT~\citep{jiang2024motiongpt} leveraged VQ-VAE~\citep{van2017neural} to discretize motion into tokens, enabling sequence modeling in the quantized space conditioned on text input.

More recently, diffusion-based approaches like MDM~\citep{tevet2023human} and Mofusion~\citep{dabral2022mofusion} adapted the denoising diffusion framework~\citep{ho2020denoising} to motion synthesis, demonstrating strong performance in multimodal scenarios including action-, text-, and music-to-motion~\citep{tseng2023edge}.

\subsection{Controlled Motion Diffusion}

The diffusion framework has proven highly adaptable, leading to numerous extensions for control and editing.
%
MDM introduced spatial and temporal editing via inpainting techniques adapted from image diffusion~\citep{saharia2022palette,song2020score}.
%
Subsequent works extended this line to propagate control signals across the denoising process for a wide range of tasks, including long-form motion generation~\citep{zhange2023diffcollage,petrovich24stmc}, in-betweening~\citep{cohan2024flexible,xie2023omnicontrol}, single-joint control~\citep{shafir2024human,karunratanakul2023gmd}, two-character interactions~\citep{shafir2024human,liang2024intergen}, and motion stylization~\citep{zhong2024smoodi,sawdayee2025dance,raab2024monkey}.
%
Alternative strategies like DNO~\citep{karunratanakul2023dno} and DartControl~\citep{Zhao:DartControl:2025} achieve more stable control by directly optimizing the initial noise vector.
%
Other works~\citep{athanasiou2023sinc,zhang2024finemogen,goel2023iterative} incorporate large language models (LLMs) to enable fine-grained control via natural language, allowing users to specify body part behaviors or pose modifiers in an intuitive interface.

Most recently, \citet{goel2025generative} and \citet{zhong2025sketch2anim} addressed the challenge of imprecise user input, both temporally and spatially, by proposing diffusion-based methods that can interpret and satisfy such loosely defined constraints.






==> spatial_tolerance.tex <==


To refine the spatial pose of input keyframes according to user-specified tolerances $\mathbf{C}$, we intervene at various steps of the inference process of  \textit{R} using a separate, unconditioned diffusion model \textit{U}. At every \textit{N} diffusion inference timesteps, in addition to generating an intermediate prediction $\tilde{\mathbf{Y}}^{R} = R(\mathbf{X}, t, \mathbf{Y}_t^{R})$, we also take a separate diffusion step on the same $\mathbf{Y}_t^{R}$ using \textit{U}, e.g., $\tilde{\mathbf{Y}}^{U} = U(t, \mathbf{Y}_t^{R})$. For each $K$ input keyposes $\mathbf{X}_{f_k}$, we identify $\tilde{\mathbf{Y}}^{U}_{f_k^*}$, where $f_k^*$ is the index of the pose in $\tilde{\mathbf{Y}}^{U}$ that is most similar to $\mathbf{X}_{f_k}$. In a standard inbetweening model that strictly preserves the timing of input keyframes, $f_k^*$ would typically equal $f_k$. However, since \textit{R} may retime keyframes during generation, $f_k^*$ need not coincide with $f_k$. In our implementation, we search within $\pm10$ frames of $f_k$ for a closest match. We then refine the keyframe pose $\mathbf{X}_{f_k}$ by blending it with the corresponding pose from the unconditioned model, weighted by the per-joint tolerance vector $\mathbf{C}_k$, i.e., $\mathbf{X}_{f_k} = \mathbf{C}_k \odot \mathbf{X}_{f_k} + (1 - \mathbf{C}_k) \odot \tilde{\mathbf{Y}}^{U}_{f_k^*}$.
where $\odot$ denotes elementwise multiplication.  We illustrate this in Fig.~\ref{fig:constraint_refinement}. High values of $\mathbf{C}$ favor greater adherence to the original keyframe; low values incorporate more of the \textit{U}'s proposal.

Our reasoning is that \textit{U} has a strong prior for plausible kinematic motion. Though $\mathbf{X}_{f_k}$ may initially be underspecified or incomplete, $\tilde{\mathbf{Y}}^{U}$ can be thought of as containing a version of $\mathbf{X}_{f_k}$ that is better aligned with \textit{U}'s learned distribution of natural looking, detailed human motion. Since $\tilde{\mathbf{Y}}^{U}$ is indirectly influenced by $\mathbf{X}$ through its dependence on $\mathbf{Y}_t^{R}$, the resulting blend remains coherent. Following each blending step, we apply IK-based postprocessing to the refined keyframes to resolve any ground penetration artifacts.


\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/keyframe_refinement/keyf_refine.png}
    \caption{\textbf{Constraint Refinement}. We simultaneously refine the input $\mathbf{X}$ to diffusion model \textit{R} while generating $\tilde{\mathbf{Y}}^{R}$. Every N timesteps, we blend input keyframes with an unconditioned proposal $\tilde{\mathbf{Y}}^{U}$ according to user-provided blending weights $\mathbf{C} \in \mathbb{R}^{K \times J}$. The resulting blended input is then used to guide subsequent inference steps of model $\mathit{R}$, and remains fixed until the next blending event. Importantly, blending modifies \textit{input keyframes} rather than the model output, avoiding the need for dense blending weights.}. 
    \label{fig:constraint_refinement}
\end{figure}


